UniAE-MoE: A Unified Audio Encoder via Mixture of Experts

Large Audio Language Models (LALMs) rely on effective audio encoders for multi-task performance. We introduce UniAE-MoE, a unified audio encoder designed to model cross-domain audio representations and achieve outstanding downstream understanding performance via a Mixture-of-Experts (MoE) architecture. Specifically, we explore mainstream audio encoders and integrate those from Qwen2-Audio and Audio-Flamingo 3, which demonstrate superior downstream capabilities. To facilitate effective model fusion, we improve our encoder using SwiGLU with shared experts to decouple encoder networks, and we further introduce a two-stage instruction-tuning strategy to better adapt the model to diverse downstream tasks. Moreover, we propose the task-specific data scaling (TSDS) technique to enhance UniAE-MoE's understanding capabilities. On the XARES-LLM benchmark, UniAE-MoE attains a score of 0.802, achieving state-of-the-art performance. It also delivers top-tier performance in the official Interspeech 2026 Audio Encoder Capability Challenge, further demonstrating robust generalization across diverse audio tasks. Together, these results validate the effectiveness of UniAE-MoE for unified audio understanding across speech, music, and general audio domains.

==> exp.tex <==
\begin{table*}[t]
    \caption{Detailed Track A results of THUVoice from Tsinghua University
    in the Interspeech 2026 Audio Encoder Capability Challenge.
    Ranks are calculated among the 23 teams listed on the official leaderboard.}
    \label{tab:thuvoice_track_a}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{4pt}
    \renewcommand{\arraystretch}{1.08}
    
    \begin{minipage}[t]{0.18\textwidth}
    \centering
    \begin{tabular}{@{}lrr@{}}
    \multicolumn{3}{c}{\textbf{Aggregate Results}}\\
    \toprule
    Result & Score & Rank\\
    \midrule
    Overall        & 0.9122 & 1\\
    Public test    & 0.8527 & 1\\
    Hidden test    & 0.9717 & 2\\
    \bottomrule
    \end{tabular}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.47\textwidth}
    \centering
    \begin{tabular}{@{}lrr@{}}
    \multicolumn{3}{c}{\textbf{Public Tasks}}\\
    \toprule
    Dataset & Score & Rank\\
    \midrule
    ASVspoof 2015          & 0.9900 & 1\\
    CREMA-D                & 0.8793 & 1\\
    ESC-50                 & 0.9125 & 5\\
    Fluent Speech Commands & 0.9939 & 5\\
    Free Music Archive     & 0.9587 & 1\\
    FSD50K                 & 0.3208 & 3\\
    FSDKaggle2018          & 0.8844 & 2\\
    GTZAN                  & 0.9091 & 3\\
    LibriCount             & 0.4790 & 10\\
    NSynth                 & 0.7881 & 1\\
    Speech Commands V1     & 0.9352 & 1\\
    UrbanSound8K           & 0.8889 & 2\\
    VocalSound             & 0.9393 & 4\\
    VoxCeleb1              & 0.9720 & 9\\
    VoxLingua33            & 0.9391 & 7\\
    \bottomrule
    \end{tabular}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.28\textwidth}
    \centering
    \begin{tabular}{@{}lrr@{}}
    \multicolumn{3}{c}{\textbf{Hidden Tasks}}\\
    \toprule
    Dataset & Score & Rank\\
    \midrule
    Fingersnap\textsuperscript{*}   & 0.8750 & 3\\
    KeyScratch\textsuperscript{*}   & 0.9990 & 1\\
    King-ASR-457\textsuperscript{*} & 0.9850 & 7\\
    King-ASR-719\textsuperscript{*} & 0.9810 & 3\\
    King-ASR-876\textsuperscript{*} & 1.0000 & 1\\
    King-ASR-955\textsuperscript{*} & 0.9900 & 1\\
    \bottomrule
    \end{tabular}
    \end{minipage}
    
    \vspace{1mm}
    \begin{minipage}{0.98\textwidth}
    \scriptsize
    \emph{Note:} The overall score is the arithmetic mean of the public-test
    and hidden-test scores. The superscript ``*'' denotes a hidden task.
    Ranks are obtained by sorting each leaderboard column in descending order;
    tied systems share the same rank.
    \end{minipage}
    \end{table*}




    \begin{table*}[t]
        \caption{Detailed Track B results of THUVoice from Tsinghua University
        in the Interspeech 2026 Audio Encoder Capability Challenge.
        Ranks are calculated among the 23 teams listed on the official leaderboard.}
        \label{tab:thuvoice_track_b}
        \centering
        \scriptsize
        \setlength{\tabcolsep}{5pt}
        \renewcommand{\arraystretch}{1.08}
        
        \begin{minipage}[t]{0.20\textwidth}
        \centering
        \begin{tabular}{@{}lrr@{}}
        \multicolumn{3}{c}{\textbf{Aggregate Results}}\\
        \toprule
        Result & Score & Rank\\
        \midrule
        Overall        & 0.6299 & 4\\
        Public test    & 0.7014 & 2\\
        Hidden test    & 0.5583 & 7\\
        \bottomrule
        \end{tabular}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.37\textwidth}
        \centering
        \begin{tabular}{@{}lrr@{}}
        \multicolumn{3}{c}{\textbf{Public Tasks}}\\
        \toprule
        Dataset & Score & Rank\\
        \midrule
        AISHELL-1       & 0.9094 & 1\\
        Clotho          & 0.4789 & 4\\
        LibriSpeech     & 0.9247 & 3\\
        MECAT           & 0.6966 & 1\\
        SongDescriber   & 0.4973 & 7\\
        \bottomrule
        \end{tabular}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.33\textwidth}
        \centering
        \begin{tabular}{@{}lrr@{}}
        \multicolumn{3}{c}{\textbf{Hidden Tasks}}\\
        \toprule
        Dataset & Score & Rank\\
        \midrule
        AISHELL-6\textsuperscript{*}  & 0.5830 & 6\\
        LibriHeavy\textsuperscript{*} & 0.7366 & 7\\
        MusicCaps\textsuperscript{*}  & 0.5155 & 1\\
        TACOS\textsuperscript{*}      & 0.3983 & 5\\
        \bottomrule
        \end{tabular}
        \end{minipage}
        
        \vspace{1mm}
        \begin{minipage}{0.98\textwidth}
        \scriptsize
        \emph{Note:} The overall score is the arithmetic mean of the public-test
        and hidden-test scores. The superscript ``*'' denotes a hidden task.
        Ranks are obtained by sorting each leaderboard column in descending order;
        tied systems share the same rank.
        \end{minipage}
        \end{table*}
